FRAIN to Train: A Fast-and-Reliable Solution for Decentralized Federated Learning

Federated learning (FL) enables collaborative model training across distributed clients while preserving data locality. Although FedAvg pioneered synchronous rounds for global model averaging, slower devices can delay collective progress. Asynchronous FL (e.g., FedAsync) addresses stragglers by continuously integrating client updates, yet naive implementations risk client drift due to non-IID data and stale contributions. Some Blockchain-based FL approaches (e.g., BRAIN) employ robust weighting or scoring of updates to resist malicious or misaligned proposals. However, performance drops can still persist under severe data heterogeneity or high staleness, and synchronization overhead has emerged as a new concern due to its aggregator-free architectures. We introduce Fast-and-Reliable AI Network, FRAIN, a new asynchronous FL method that mitigates these limitations by incorporating two key ideas. First, our FastSync strategy eliminates the need to replay past model versions, enabling newcomers and infrequent participants to efficiently approximate the global model. Second, we adopt spherical linear interpolation (SLERP) when merging parameters, preserving models' directions and alleviating destructive interference from divergent local training. Experiments with a CNN image-classification model and a Transformer-based language model demonstrate that FRAIN achieves more stable and robust convergence than FedAvg, FedAsync, and BRAIN, especially under harsh environments: non-IID data distributions, networks that experience delays and require frequent re-synchronization, and the presence of malicious nodes.

==> algorithms/fastsync.tex <==
\begin{algorithm}[!th]
\caption{\textsc{FastSync}: Rapid Approximation of the Global Model from Recent Proposals}
\label{algo:fastsync}
\begin{algorithmic}[1]

\Require $\text{current round } r \ge 1$, 
\Statex $\quad \text{look-back window } N \ge 2$,
\Statex $\quad \text{proposal set } \{(M_{r-k}, \alpha_{r-k}) \mid k = 0,1,\dots,N-1\}$,
\Statex $\quad \text{threshold } \mathcal{T} \text{ where } 0 \le \mathcal{T} < 1$.
\Ensure $\textit{pseudo-global model} \overline{M}_r^\prime \text{ computed via FastSync}$.

\vspace{0.3em}
\Procedure{FastSync}{$N, r$}
    \State \textbf{initialize:} $\mathcal{W} \gets 0,\quad \overline{M}_r^\prime \gets \mathbf{0}$
    \Comment{accumulators for weight sum and weighted sum}
    \For{$k$ in $0$ to $N-1$}
        \State \textbf{let} $(M_{r-k},\, \alpha_{r-k})$ \text{ be the $k$-th most recent proposal}
        \If {$\alpha_{r-k} \;\ge\; \mathcal{T}$}
            \Comment{only consider proposals above threshold}
            \State $\overline{M}_r^\prime \;\gets\; \overline{M}_r^\prime \;+\; \alpha_{r-k}\,M_{r-k}$
            \State $\mathcal{W} \;\gets\; \mathcal{W} \;+\; \alpha_{r-k}$
        \EndIf
    \EndFor
    \If {$\mathcal{W} > 0$}
        \State $\overline{M}_r^\prime \;\gets\; \frac{\overline{M}_r^\prime}{\mathcal{W}}$
        \Comment{final weighted linear blend}
    \Else
        \State \textbf{fallback:} $\overline{M}_r^\prime \;\gets\; \mathbf{0} \quad$ 
        \Comment{or some default model if no valid proposals remain}
    \EndIf
    \State \Return $\overline{M}_r^\prime$
\EndProcedure

\end{algorithmic}
\end{algorithm}


==> texts/experiments/_sync.tex <==
\input{graphs/sync}


\subsection{SYNCHRONIZATION} \label{subsection:experiment-sync}


In the {\em Fast Sync} approach, nodes join without calculating a global model, leading to updates that may deviate from the ideal global model.
To evaluate the impact of these drifted proposals, we conducted experiments with various numbers of drifted nodes, relative to a total of 21 nodes.
These nodes do train based on a global-like model calculated through Fast Sync and then make new proposals.

The results, illustrated in Fig.~\ref{fig:drift}, show that even with a significant number of drifted nodes, performance remains stable under both IID and non-IID conditions.
Notably, in scenarios where all 21 nodes are drifted, meaning all participating nodes exclusively employ the Fast Sync method without reference to a global model, no performance degradation is observed.


==> texts/experiments/staleness.tex <==
% \subsection{Effect of Staleness}
% \label{subsec:staleness}

% In Figure~\ref{fig:stale_accuracy}, we vary the degree of staleness to examine how each method copes with delayed updates. Staleness levels range from minimal delay (\(=0\)) to severe delay (\(=4\)):
% \begin{itemize}
%     \item \textbf{FedAsync} performance drops sharply as staleness increases, likely due to naive immediate integration of outdated models.
%     \item \textbf{BRAIN} fares better by filtering low-scoring proposals, but still shows some instability under high staleness.
%     \item \textbf{FRAIN} consistently maintains higher accuracy. Its hinge-based $\alpha$ function penalizes old proposals more aggressively, while SLERP merging prevents destructive interference from delayed updates.
% \end{itemize}


==> texts/related_work/fastsync.tex <==
\subsection{Client Drift}
\label{subsec:client_drift}

A prominent line of research tackles {client drift}---where local models diverge from the global objective due to non-IID data, stale updates, or extended local training.
%
For instance, \textit{FedProx}~\cite{fedprox} introduces a proximal term that regularizes each local objective, preventing local updates from straying too far from the current global model. This approach alleviates drift in synchronous FL with non-IID data.
%
\textit{SCAFFOLD}~\cite{scaffold} sends {control variates} from the server to each client, correcting local updates and reducing drift.
%    
\textit{FedAsync}~\cite{fedasync} proposes to adjust the interpolation coefficient \(\alpha\) based on how stale each update is. 


% \bigskip
% \noindent
% \textbf{Comparison to FRAIN.}


FRAIN also aims to mitigate client drift, particularly in the presence of non-IID data.
However, FRAIN’s integration is inherently {asynchronous} and decentralized, meaning it must handle both client delays and potential Byzantine behaviors.
%
Both FedProx and SCAFFOLD primarily address synchronous FL scenarios; they do not explicitly handle the {stale} updates that arise in asynchronous settings.
%
%
Inspired from FedAsync, FRAIN also adjusts \(\alpha\) to manage staleness, but it goes further by:
Employing a {score-based} filter to penalize or discard proposals that appear to be malicious or excessively stale; and
Introducing {SLERP-based merging} to preserve directional information and reduce destructive interference.
%
%
Thus, FRAIN addresses both drift and adversarial threats under realistic asynchronous conditions, which distinguishes it from prior synchronous solutions.


==> texts/related_work/slerp.tex <==
\subsection{SLERP and Non-Linear Interpolation}
\label{subsec:slerp_related}

Recent studies have explored improved {non-linear} interpolation strategies for federated or distributed training. Linear averaging (FedAvg) can trap updates in {loss barriers} when the parameter vectors point in conflicting directions, especially under significant data heterogeneity or staleness.
%
% \paragraph{AsyncManifold.}
\textit{AsyncManifold}~\cite{asyncmanifold} highlights that asynchronous FL with {stale} and {highly heterogeneous} clients can suffer from steep performance drops if updates are naively merged. They propose a geometric approach on manifolds, along with an {OrthoCorrect} mechanism to project out the conflicting component of outdated updates. 
%
%
% TODO: 방향 검증은 불가능 컨트랙트상에서


% \bigskip
% \noindent
% \textbf{Comparison to FRAIN.}


FRAIN likewise draws on the idea of {spherical} interpolation to handle divergent model updates. Unlike AsyncManifold’s OrthoCorrect, which modifies each gradient in a multi-step process, FRAIN focuses on aggregator-free {score-based} weighting to remain blockchain-compatible. Specifically:
%
\begin{itemize}
    \item FRAIN uses {SLERP} {post hoc} on the global model side, guided by a \(\alpha\) score computed from on-chain data (instead of each node modifying its own update).
    
    \item The overhead stays modest, as we only store and verify {scores} on-chain, not full gradient vectors. This enables FRAIN to scale to extremely large networks and model sizes in a decentralized manner, without the high cost of verifying each update direction on-chain.
    While OrthoCorrect can effectively disentangle directions of conflicting gradients, it requires more complex {client-side} adjustments and cannot trivially be validated on-chain in a decentralized setting.
\end{itemize}
%
Thus, while FRAIN shares the conceptual thread of “geometric merging” with AsyncManifold and MergeKit, it is uniquely tailored to {asynchronous, blockchain-based FL}, leveraging simpler score mechanisms suitable for on-chain consensus.
%
This balance of practical feasibility and robust geometric interpolation differentiates FRAIN from existing methods.

